Probing Ranking LLMs: A Mechanistic Analysis for Information Retrieval

Transformer networks, particularly those achieving performance comparable to GPT models, are well known for their robust feature extraction abilities. However, the nature of these extracted features and their alignment with human-engineered ones remain unexplored. In this work, we investigate the internal mechanisms of state-of-the-art, fine-tuned LLMs for passage reranking. We employ a probing-based analysis to examine neuron activations in ranking LLMs, identifying the presence of known human-engineered and semantic features. Our study spans a broad range of feature categories, including lexical signals, document structure, query-document interactions, and complex semantic representations, to uncover underlying patterns influencing ranking decisions. Through experiments on four different ranking LLMs, we identify statistical IR features that are prominently encoded in LLM activations, as well as others that are notably missing. Furthermore, we analyze how these models respond to out-of-distribution queries and documents, revealing distinct generalization behaviors. By dissecting the latent representations within LLM activations, we aim to improve both the interpretability and effectiveness of ranking models. Our findings offer crucial insights for developing more transparent and reliable retrieval systems, and we release all necessary scripts and code to support further exploration.

==> SIGIR25/removed_data.tex <==
@article{sajjad2022neuron,
  title={Neuron-level interpretation of deep nlp models: A survey},
  author={Sajjad, Hassan and Durrani, Nadir and Dalvi, Fahim},
  journal={Transactions of the Association for Computational Linguistics},
  volume={10},
  pages={1285--1303},
  year={2022},
  publisher={MIT Press One Broadway, 12th Floor, Cambridge, Massachusetts 02142, USA~…}
}

@article{ma2023fine,
  title={Fine-tuning llama for multi-stage text retrieval},
  author={Ma, Xueguang and Wang, Liang and Yang, Nan and Wei, Furu and Lin, Jimmy},
  journal={arXiv preprint arXiv:2310.08319},
  year={2023}
}

@article{gurnee2023finding,
  title={Finding neurons in a haystack: Case studies with sparse probing},
  author={Gurnee, Wes and Nanda, Neel and Pauly, Matthew and Harvey, Katherine and Troitskii, Dmitrii and Bertsimas, Dimitris},
  journal={arXiv preprint arXiv:2305.01610},
  year={2023}
}

@inproceedings{rauker2023toward,
  title={Toward transparent ai: A survey on interpreting the inner structures of deep neural networks},
  author={R{\"a}uker, Tilman and Ho, Anson and Casper, Stephen and Hadfield-Menell, Dylan},
  booktitle={2023 IEEE Conference on Secure and Trustworthy Machine Learning (SaTML)},
  pages={464--483},
  year={2023},
  organization={IEEE}
}

@article{geva2020transformer,
  title={Transformer feed-forward layers are key-value memories},
  author={Geva, Mor and Schuster, Roei and Berant, Jonathan and Levy, Omer},
  journal={arXiv preprint arXiv:2012.14913},
  year={2020}
}

@article{geva2022transformer,
  title={Transformer feed-forward layers build predictions by promoting concepts in the vocabulary space},
  author={Geva, Mor and Caciularu, Avi and Wang, Kevin Ro and Goldberg, Yoav},
  journal={arXiv preprint arXiv:2203.14680},
  year={2022}
}

@article{belinkov2022probing,
  title={Probing classifiers: Promises, shortcomings, and advances},
  author={Belinkov, Yonatan},
  journal={Computational Linguistics},
  volume={48},
  number={1},
  pages={207--219},
  year={2022},
  publisher={MIT Press One Broadway, 12th Floor, Cambridge, Massachusetts 02142, USA~…}
}

@inproceedings{de2019bias,
  title={Bias in bios: A case study of semantic representation bias in a high-stakes setting},
  author={De-Arteaga, Maria and Romanov, Alexey and Wallach, Hanna and Chayes, Jennifer and Borgs, Christian and Chouldechova, Alexandra and Geyik, Sahin and Kenthapadi, Krishnaram and Kalai, Adam Tauman},
  booktitle={proceedings of the Conference on Fairness, Accountability, and Transparency},
  pages={120--128},
  year={2019}
}

@article{csordas2020neural,
  title={Are neural nets modular? inspecting functional modularity through differentiable weight masks},
  author={Csord{\'a}s, R{\'o}bert and van Steenkiste, Sjoerd and Schmidhuber, J{\"u}rgen},
  journal={arXiv preprint arXiv:2010.02066},
  year={2020}
}

@article{wortsman2020supermasks,
  title={Supermasks in superposition},
  author={Wortsman, Mitchell and Ramanujan, Vivek and Liu, Rosanne and Kembhavi, Aniruddha and Rastegari, Mohammad and Yosinski, Jason and Farhadi, Ali},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={15173--15184},
  year={2020}
}

@article{zhou2014object,
  title={Object detectors emerge in deep scene cnns},
  author={Zhou, Bolei and Khosla, Aditya and Lapedriza, Agata and Oliva, Aude and Torralba, Antonio},
  journal={arXiv preprint arXiv:1412.6856},
  year={2014}
}

@article{ancona2019gradient,
  title={Gradient-based attribution methods},
  author={Ancona, Marco and Ceolini, Enea and {\"O}ztireli, Cengiz and Gross, Markus},
  journal={Explainable AI: Interpreting, explaining and visualizing deep learning},
  pages={169--191},
  year={2019},
  publisher={Springer}
}

@article{zhou2018revisiting,
  title={Revisiting the importance of individual units in cnns via ablation},
  author={Zhou, Bolei and Sun, Yiyou and Bau, David and Torralba, Antonio},
  journal={arXiv preprint arXiv:1806.02891},
  year={2018}
}

@article{meister2021sparse,
  title={Is sparse attention more interpretable?},
  author={Meister, Clara and Lazov, Stefan and Augenstein, Isabelle and Cotterell, Ryan},
  journal={arXiv preprint arXiv:2106.01087},
  year={2021}
}

@inproceedings{fiacco2019deep,
  title={Deep neural model inspection and comparison via functional neuron pathways},
  author={Fiacco, James and Choudhary, Samridhi and Rose, Carolyn},
  booktitle={Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics},
  pages={5754--5764},
  year={2019}
}

@article{clark2019does,
  title={What does bert look at? an analysis of bert's attention},
  author={Clark, Kevin and Khandelwal, Urvashi and Levy, Omer and Manning, Christopher D},
  journal={arXiv preprint arXiv:1906.04341},
  year={2019}
}

@article{li2021implicit,
  title={Implicit representations of meaning in neural language models},
  author={Li, Belinda Z and Nye, Maxwell and Andreas, Jacob},
  journal={arXiv preprint arXiv:2106.00737},
  year={2021}
}

@article{ravichander2020probing,
  title={Probing the probing paradigm: Does probing accuracy entail task relevance?},
  author={Ravichander, Abhilasha and Belinkov, Yonatan and Hovy, Eduard},
  journal={arXiv preprint arXiv:2005.00719},
  year={2020}
}



@inproceedings{chowdhury2023rank,
  title={Rank-lime: local model-agnostic feature attribution for learning to rank},
  author={Chowdhury, Tanya and Rahimi, Razieh and Allan, James},
  booktitle={Proceedings of the 2023 ACM SIGIR International Conference on Theory of Information Retrieval},
  pages={33--37},
  year={2023}
}

@article{anand2022explainable,
  title={Explainable information retrieval: A survey},
  author={Anand, Avishek and Lyu, Lijun and Idahl, Maximilian and Wang, Yumeng and Wallat, Jonas and Zhang, Zijian},
  journal={arXiv preprint arXiv:2211.02405},
  year={2022}
}

@inproceedings{zhan2020analysis,
  title={An analysis of BERT in document ranking},
  author={Zhan, Jingtao and Mao, Jiaxin and Liu, Yiqun and Zhang, Min and Ma, Shaoping},
  booktitle={Proceedings of the 43rd International ACM SIGIR conference on research and development in Information Retrieval},
  pages={1941--1944},
  year={2020}
}

@article{choi2022finding,
  title={Finding Inverse Document Frequency Information in BERT},
  author={Choi, Jaekeol and Jung, Euna and Lim, Sungjun and Rhee, Wonjong},
  journal={arXiv preprint arXiv:2202.12191},
  year={2022}
}

@inproceedings{formal2021white,
  title={A white box analysis of ColBERT},
  author={Formal, Thibault and Piwowarski, Benjamin and Clinchant, St{\'e}phane},
  booktitle={Advances in Information Retrieval: 43rd European Conference on IR Research, ECIR 2021, Virtual Event, March 28--April 1, 2021, Proceedings, Part II 43},
  pages={257--263},
  year={2021},
  organization={Springer}
}

@inproceedings{formal2022match,
  title={Match your words! a study of lexical matching in neural information retrieval},
  author={Formal, Thibault and Piwowarski, Benjamin and Clinchant, St{\'e}phane},
  booktitle={European Conference on Information Retrieval},
  pages={120--127},
  year={2022},
  organization={Springer}
}

@article{elhage2021mathematical,
  title={A mathematical framework for transformer circuits},
  author={Elhage, Nelson and Nanda, Neel and Olsson, Catherine and Henighan, Tom and Joseph, Nicholas and Mann, Ben and Askell, Amanda and Bai, Yuntao and Chen, Anna and Conerly, Tom and others},
  journal={Transformer Circuits Thread},
  volume={1},
  pages={1},
  year={2021}
}

@article{DBLP:journals/corr/QinL13,
  author    = {Tao Qin and
               Tie{-}Yan Liu},
  title     = {Introducing {LETOR} 4.0 Datasets},
  journal   = {CoRR},
  volume    = {abs/1306.2597},
  year      = {2013},
  url       = {http://arxiv.org/abs/1306.2597},
  timestamp = {Mon, 01 Jul 2013 20:31:25 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/QinL13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{bau2020understanding,
  title={Understanding the role of individual units in a deep neural network},
  author={Bau, David and Zhu, Jun-Yan and Strobelt, Hendrik and Lapedriza, Agata and Zhou, Bolei and Torralba, Antonio},
  journal={Proceedings of the National Academy of Sciences},
  volume={117},
  number={48},
  pages={30071--30078},
  year={2020},
  publisher={National Acad Sciences}
}

@inproceedings{chen2024axiomatic,
  title={Axiomatic Causal Interventions for Reverse Engineering Relevance Computation in Neural Retrieval Models},
  author={Chen, Catherine and Merullo, Jack and Eickhoff, Carsten},
  booktitle={Proceedings of the 47th International ACM SIGIR Conference on Research and Development in Information Retrieval},
  pages={1401--1410},
  year={2024}
}


@inproceedings{wallat2023probing,
  title={Probing BERT for ranking abilities},
  author={Wallat, Jonas and Beringer, Fabian and Anand, Abhijit and Anand, Avishek},
  booktitle={European Conference on Information Retrieval},
  pages={255--273},
  year={2023},
  organization={Springer}
}

@inproceedings{vast2024neurons,
  title={Which Neurons Matter in IR? Applying Integrated Gradients-based Methods to Understand Cross-Encoders},
  author={Vast, Mathias and Van Cooten, Basile and Soulier, Laure and Piwowarski, Benjamin},
  booktitle={Proceedings of the 2024 ACM SIGIR International Conference on Theory of Information Retrieval},
  pages={133--143},
  year={2024}
}

@article{macavaney2022abnirml,
  title={ABNIRML: Analyzing the behavior of neural IR models},
  author={MacAvaney, Sean and Feldman, Sergey and Goharian, Nazli and Downey, Doug and Cohan, Arman},
  journal={Transactions of the Association for Computational Linguistics},
  volume={10},
  pages={224--239},
  year={2022},
  publisher={MIT Press One Broadway, 12th Floor, Cambridge, Massachusetts 02142 journals~…}
}

@inproceedings{fan2021linguistic,
  title={A linguistic study on relevance modeling in information retrieval},
  author={Fan, Yixing and Guo, Jiafeng and Ma, Xinyu and Zhang, Ruqing and Lan, Yanyan and Cheng, Xueqi},
  booktitle={Proceedings of the Web Conference 2021},
  pages={1053--1064},
  year={2021}
}

@inproceedings{fernando2019study,
  title={A study on the Interpretability of Neural Retrieval Models using DeepSHAP},
  author={Fernando, Zeon Trevor and Singh, Jaspreet and Anand, Avishek},
  booktitle={Proceedings of the 42nd international ACM SIGIR conference on research and development in information retrieval},
  pages={1005--1008},
  year={2019}
}

@article{thakur2021beir,
  title={Beir: A heterogenous benchmark for zero-shot evaluation of information retrieval models},
  author={Thakur, Nandan and Reimers, Nils and R{\"u}ckl{\'e}, Andreas and Srivastava, Abhishek and Gurevych, Iryna},
  journal={arXiv preprint arXiv:2104.08663},
  year={2021}
}

@online{h4stackexchange,
  author = {Lambert, Nathan and Tunstall, Lewis and Rajani, Nazneen and Thrush, Tristan},
  title = {HuggingFace H4 Stack Exchange Preference Dataset},
  year = 2023,
  url = {https://huggingface.co/datasets/HuggingFaceH4/stack-exchange-preferences},
}

@inproceedings{khattab2020colbert,
  title={Colbert: Efficient and effective passage search via contextualized late interaction over bert},
  author={Khattab, Omar and Zaharia, Matei},
  booktitle={Proceedings of the 43rd International ACM SIGIR conference on research and development in Information Retrieval},
  pages={39--48},
  year={2020}
}

@article{han2018feature,
  title={Feature selection and model comparison on microsoft learning-to-rank data sets},
  author={Han, Xinzhi and Lei, Sen},
  journal={arXiv preprint arXiv:1803.05127},
  year={2018}
}

@article{hochma2024efficient,
  title={Efficient Feature Ranking and Selection using Statistical Moments},
  author={Hochma, Yael and Felendler, Yuval and Last, Mark},
  journal={IEEE Access},
  year={2024},
  publisher={IEEE}
}

@article{nguyen2016ms,
  title={Ms marco: A human-generated machine reading comprehension dataset},
  author={Nguyen, Tri and Rosenberg, Mir and Song, Xia and Gao, Jianfeng and Tiwary, Saurabh and Majumder, Rangan and Deng, Li},
  year={2016}
}

@article{chowdhury2024rankshap,
  title={RankSHAP: a Gold Standard Feature Attribution Method for the Ranking Task},
  author={Chowdhury, Tanya and Zick, Yair and Allan, James},
  journal={arXiv preprint arXiv:2405.01848},
  year={2024}
}

@inproceedings{shrikumar2017learning,
  title={Learning important features through propagating activation differences},
  author={Shrikumar, Avanti and Greenside, Peyton and Kundaje, Anshul},
  booktitle={International conference on machine learning},
  pages={3145--3153},
  year={2017},
  organization={PMlR}
}

@article{lundberg2017unified,
  title={A unified approach to interpreting model predictions},
  author={Lundberg, Scott M and Lee, Su-In},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@inproceedings{sundararajan2020many,
  title={The many Shapley values for model explanation},
  author={Sundararajan, Mukund and Najmi, Amir},
  booktitle={International conference on machine learning},
  pages={9269--9278},
  year={2020},
  organization={PMLR}
}

==> removed_data.tex <==
@article{sajjad2022neuron,
  title={Neuron-level interpretation of deep nlp models: A survey},
  author={Sajjad, Hassan and Durrani, Nadir and Dalvi, Fahim},
  journal={Transactions of the Association for Computational Linguistics},
  volume={10},
  pages={1285--1303},
  year={2022},
  publisher={MIT Press One Broadway, 12th Floor, Cambridge, Massachusetts 02142, USA~…}
}

@article{ma2023fine,
  title={Fine-tuning llama for multi-stage text retrieval},
  author={Ma, Xueguang and Wang, Liang and Yang, Nan and Wei, Furu and Lin, Jimmy},
  journal={arXiv preprint arXiv:2310.08319},
  year={2023}
}

@article{gurnee2023finding,
  title={Finding neurons in a haystack: Case studies with sparse probing},
  author={Gurnee, Wes and Nanda, Neel and Pauly, Matthew and Harvey, Katherine and Troitskii, Dmitrii and Bertsimas, Dimitris},
  journal={arXiv preprint arXiv:2305.01610},
  year={2023}
}

@inproceedings{rauker2023toward,
  title={Toward transparent ai: A survey on interpreting the inner structures of deep neural networks},
  author={R{\"a}uker, Tilman and Ho, Anson and Casper, Stephen and Hadfield-Menell, Dylan},
  booktitle={2023 IEEE Conference on Secure and Trustworthy Machine Learning (SaTML)},
  pages={464--483},
  year={2023},
  organization={IEEE}
}

@article{geva2020transformer,
  title={Transformer feed-forward layers are key-value memories},
  author={Geva, Mor and Schuster, Roei and Berant, Jonathan and Levy, Omer},
  journal={arXiv preprint arXiv:2012.14913},
  year={2020}
}

@article{geva2022transformer,
  title={Transformer feed-forward layers build predictions by promoting concepts in the vocabulary space},
  author={Geva, Mor and Caciularu, Avi and Wang, Kevin Ro and Goldberg, Yoav},
  journal={arXiv preprint arXiv:2203.14680},
  year={2022}
}

@article{belinkov2022probing,
  title={Probing classifiers: Promises, shortcomings, and advances},
  author={Belinkov, Yonatan},
  journal={Computational Linguistics},
  volume={48},
  number={1},
  pages={207--219},
  year={2022},
  publisher={MIT Press One Broadway, 12th Floor, Cambridge, Massachusetts 02142, USA~…}
}

@inproceedings{de2019bias,
  title={Bias in bios: A case study of semantic representation bias in a high-stakes setting},
  author={De-Arteaga, Maria and Romanov, Alexey and Wallach, Hanna and Chayes, Jennifer and Borgs, Christian and Chouldechova, Alexandra and Geyik, Sahin and Kenthapadi, Krishnaram and Kalai, Adam Tauman},
  booktitle={proceedings of the Conference on Fairness, Accountability, and Transparency},
  pages={120--128},
  year={2019}
}

@article{csordas2020neural,
  title={Are neural nets modular? inspecting functional modularity through differentiable weight masks},
  author={Csord{\'a}s, R{\'o}bert and van Steenkiste, Sjoerd and Schmidhuber, J{\"u}rgen},
  journal={arXiv preprint arXiv:2010.02066},
  year={2020}
}

@article{wortsman2020supermasks,
  title={Supermasks in superposition},
  author={Wortsman, Mitchell and Ramanujan, Vivek and Liu, Rosanne and Kembhavi, Aniruddha and Rastegari, Mohammad and Yosinski, Jason and Farhadi, Ali},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={15173--15184},
  year={2020}
}

@article{zhou2014object,
  title={Object detectors emerge in deep scene cnns},
  author={Zhou, Bolei and Khosla, Aditya and Lapedriza, Agata and Oliva, Aude and Torralba, Antonio},
  journal={arXiv preprint arXiv:1412.6856},
  year={2014}
}

@article{ancona2019gradient,
  title={Gradient-based attribution methods},
  author={Ancona, Marco and Ceolini, Enea and {\"O}ztireli, Cengiz and Gross, Markus},
  journal={Explainable AI: Interpreting, explaining and visualizing deep learning},
  pages={169--191},
  year={2019},
  publisher={Springer}
}

@article{zhou2018revisiting,
  title={Revisiting the importance of individual units in cnns via ablation},
  author={Zhou, Bolei and Sun, Yiyou and Bau, David and Torralba, Antonio},
  journal={arXiv preprint arXiv:1806.02891},
  year={2018}
}

@article{meister2021sparse,
  title={Is sparse attention more interpretable?},
  author={Meister, Clara and Lazov, Stefan and Augenstein, Isabelle and Cotterell, Ryan},
  journal={arXiv preprint arXiv:2106.01087},
  year={2021}
}

@inproceedings{fiacco2019deep,
  title={Deep neural model inspection and comparison via functional neuron pathways},
  author={Fiacco, James and Choudhary, Samridhi and Rose, Carolyn},
  booktitle={Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics},
  pages={5754--5764},
  year={2019}
}

@article{clark2019does,
  title={What does bert look at? an analysis of bert's attention},
  author={Clark, Kevin and Khandelwal, Urvashi and Levy, Omer and Manning, Christopher D},
  journal={arXiv preprint arXiv:1906.04341},
  year={2019}
}

@article{li2021implicit,
  title={Implicit representations of meaning in neural language models},
  author={Li, Belinda Z and Nye, Maxwell and Andreas, Jacob},
  journal={arXiv preprint arXiv:2106.00737},
  year={2021}
}

@article{ravichander2020probing,
  title={Probing the probing paradigm: Does probing accuracy entail task relevance?},
  author={Ravichander, Abhilasha and Belinkov, Yonatan and Hovy, Eduard},
  journal={arXiv preprint arXiv:2005.00719},
  year={2020}
}



@inproceedings{chowdhury2023rank,
  title={Rank-lime: local model-agnostic feature attribution for learning to rank},
  author={Chowdhury, Tanya and Rahimi, Razieh and Allan, James},
  booktitle={Proceedings of the 2023 ACM SIGIR International Conference on Theory of Information Retrieval},
  pages={33--37},
  year={2023}
}

@article{anand2022explainable,
  title={Explainable information retrieval: A survey},
  author={Anand, Avishek and Lyu, Lijun and Idahl, Maximilian and Wang, Yumeng and Wallat, Jonas and Zhang, Zijian},
  journal={arXiv preprint arXiv:2211.02405},
  year={2022}
}

@inproceedings{zhan2020analysis,
  title={An analysis of BERT in document ranking},
  author={Zhan, Jingtao and Mao, Jiaxin and Liu, Yiqun and Zhang, Min and Ma, Shaoping},
  booktitle={Proceedings of the 43rd International ACM SIGIR conference on research and development in Information Retrieval},
  pages={1941--1944},
  year={2020}
}

@article{choi2022finding,
  title={Finding Inverse Document Frequency Information in BERT},
  author={Choi, Jaekeol and Jung, Euna and Lim, Sungjun and Rhee, Wonjong},
  journal={arXiv preprint arXiv:2202.12191},
  year={2022}
}

@inproceedings{formal2021white,
  title={A white box analysis of ColBERT},
  author={Formal, Thibault and Piwowarski, Benjamin and Clinchant, St{\'e}phane},
  booktitle={Advances in Information Retrieval: 43rd European Conference on IR Research, ECIR 2021, Virtual Event, March 28--April 1, 2021, Proceedings, Part II 43},
  pages={257--263},
  year={2021},
  organization={Springer}
}

@inproceedings{formal2022match,
  title={Match your words! a study of lexical matching in neural information retrieval},
  author={Formal, Thibault and Piwowarski, Benjamin and Clinchant, St{\'e}phane},
  booktitle={European Conference on Information Retrieval},
  pages={120--127},
  year={2022},
  organization={Springer}
}

@article{elhage2021mathematical,
  title={A mathematical framework for transformer circuits},
  author={Elhage, Nelson and Nanda, Neel and Olsson, Catherine and Henighan, Tom and Joseph, Nicholas and Mann, Ben and Askell, Amanda and Bai, Yuntao and Chen, Anna and Conerly, Tom and others},
  journal={Transformer Circuits Thread},
  volume={1},
  pages={1},
  year={2021}
}

@article{DBLP:journals/corr/QinL13,
  author    = {Tao Qin and
               Tie{-}Yan Liu},
  title     = {Introducing {LETOR} 4.0 Datasets},
  journal   = {CoRR},
  volume    = {abs/1306.2597},
  year      = {2013},
  url       = {http://arxiv.org/abs/1306.2597},
  timestamp = {Mon, 01 Jul 2013 20:31:25 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/QinL13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{bau2020understanding,
  title={Understanding the role of individual units in a deep neural network},
  author={Bau, David and Zhu, Jun-Yan and Strobelt, Hendrik and Lapedriza, Agata and Zhou, Bolei and Torralba, Antonio},
  journal={Proceedings of the National Academy of Sciences},
  volume={117},
  number={48},
  pages={30071--30078},
  year={2020},
  publisher={National Acad Sciences}
}

@inproceedings{chen2024axiomatic,
  title={Axiomatic Causal Interventions for Reverse Engineering Relevance Computation in Neural Retrieval Models},
  author={Chen, Catherine and Merullo, Jack and Eickhoff, Carsten},
  booktitle={Proceedings of the 47th International ACM SIGIR Conference on Research and Development in Information Retrieval},
  pages={1401--1410},
  year={2024}
}


@inproceedings{wallat2023probing,
  title={Probing BERT for ranking abilities},
  author={Wallat, Jonas and Beringer, Fabian and Anand, Abhijit and Anand, Avishek},
  booktitle={European Conference on Information Retrieval},
  pages={255--273},
  year={2023},
  organization={Springer}
}

@inproceedings{vast2024neurons,
  title={Which Neurons Matter in IR? Applying Integrated Gradients-based Methods to Understand Cross-Encoders},
  author={Vast, Mathias and Van Cooten, Basile and Soulier, Laure and Piwowarski, Benjamin},
  booktitle={Proceedings of the 2024 ACM SIGIR International Conference on Theory of Information Retrieval},
  pages={133--143},
  year={2024}
}

@article{macavaney2022abnirml,
  title={ABNIRML: Analyzing the behavior of neural IR models},
  author={MacAvaney, Sean and Feldman, Sergey and Goharian, Nazli and Downey, Doug and Cohan, Arman},
  journal={Transactions of the Association for Computational Linguistics},
  volume={10},
  pages={224--239},
  year={2022},
  publisher={MIT Press One Broadway, 12th Floor, Cambridge, Massachusetts 02142 journals~…}
}

@inproceedings{fan2021linguistic,
  title={A linguistic study on relevance modeling in information retrieval},
  author={Fan, Yixing and Guo, Jiafeng and Ma, Xinyu and Zhang, Ruqing and Lan, Yanyan and Cheng, Xueqi},
  booktitle={Proceedings of the Web Conference 2021},
  pages={1053--1064},
  year={2021}
}

@inproceedings{fernando2019study,
  title={A study on the Interpretability of Neural Retrieval Models using DeepSHAP},
  author={Fernando, Zeon Trevor and Singh, Jaspreet and Anand, Avishek},
  booktitle={Proceedings of the 42nd international ACM SIGIR conference on research and development in information retrieval},
  pages={1005--1008},
  year={2019}
}

@article{thakur2021beir,
  title={Beir: A heterogenous benchmark for zero-shot evaluation of information retrieval models},
  author={Thakur, Nandan and Reimers, Nils and R{\"u}ckl{\'e}, Andreas and Srivastava, Abhishek and Gurevych, Iryna},
  journal={arXiv preprint arXiv:2104.08663},
  year={2021}
}

@online{h4stackexchange,
  author = {Lambert, Nathan and Tunstall, Lewis and Rajani, Nazneen and Thrush, Tristan},
  title = {HuggingFace H4 Stack Exchange Preference Dataset},
  year = 2023,
  url = {https://huggingface.co/datasets/HuggingFaceH4/stack-exchange-preferences},
}

@inproceedings{khattab2020colbert,
  title={Colbert: Efficient and effective passage search via contextualized late interaction over bert},
  author={Khattab, Omar and Zaharia, Matei},
  booktitle={Proceedings of the 43rd International ACM SIGIR conference on research and development in Information Retrieval},
  pages={39--48},
  year={2020}
}

@article{han2018feature,
  title={Feature selection and model comparison on microsoft learning-to-rank data sets},
  author={Han, Xinzhi and Lei, Sen},
  journal={arXiv preprint arXiv:1803.05127},
  year={2018}
}

@article{hochma2024efficient,
  title={Efficient Feature Ranking and Selection using Statistical Moments},
  author={Hochma, Yael and Felendler, Yuval and Last, Mark},
  journal={IEEE Access},
  year={2024},
  publisher={IEEE}
}

@article{nguyen2016ms,
  title={Ms marco: A human-generated machine reading comprehension dataset},
  author={Nguyen, Tri and Rosenberg, Mir and Song, Xia and Gao, Jianfeng and Tiwary, Saurabh and Majumder, Rangan and Deng, Li},
  year={2016}
}

@article{chowdhury2024rankshap,
  title={RankSHAP: a Gold Standard Feature Attribution Method for the Ranking Task},
  author={Chowdhury, Tanya and Zick, Yair and Allan, James},
  journal={arXiv preprint arXiv:2405.01848},
  year={2024}
}

@inproceedings{shrikumar2017learning,
  title={Learning important features through propagating activation differences},
  author={Shrikumar, Avanti and Greenside, Peyton and Kundaje, Anshul},
  booktitle={International conference on machine learning},
  pages={3145--3153},
  year={2017},
  organization={PMlR}
}

@article{lundberg2017unified,
  title={A unified approach to interpreting model predictions},
  author={Lundberg, Scott M and Lee, Su-In},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@inproceedings{sundararajan2020many,
  title={The many Shapley values for model explanation},
  author={Sundararajan, Mukund and Najmi, Amir},
  booktitle={International conference on machine learning},
  pages={9269--9278},
  year={2020},
  organization={PMLR}
}
